Infinite Choice and Probability Distributions. An Open Problem: The Real Hotel

We sketch a process algebra with data and probability distributions. This allows to combine two very powerful abstraction mechanisms namely non-deterministic choice and probabilities. However, it is not clear how to define an appropriate semantics for the generalised choice over data in combination with probability density functions. The real hotel is a puzzle that exemplifies the core of the problem.

==> eptcsdata.tex <==
\providecommand{\firstpage}{2}
\providecommand{\publicationstatus}{V. Castiglioni and O. Dardha (Eds.): Combined Workshop on \\Expressiveness in Concurrency and Structural Operational Semantics \\ (EXPRESS/SOS 2021)\\
EPTCS 339, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.339.2}{10.4204/EPTCS.339.2}}

